Towards an Interpretable Latent Space in Structured Models for Video Prediction

We focus on the task of future frame prediction in video governed by underlying physical dynamics. We work with models which are object-centric, i.e., explicitly work with object representations, and propagate a loss in the latent space. Specifically, our research builds on recent work by Kipf et al. \cite{kipf&al20}, which predicts the next state via contrastive learning of object interactions in a latent space using a Graph Neural Network. We argue that injecting explicit inductive bias in the model, in form of general physical laws, can help not only make the model more interpretable, but also improve the overall prediction of model. As a natural by-product, our model can learn feature maps which closely resemble actual object positions in the image, without having any explicit supervision about the object positions at the training time. In comparison with earlier works \cite{jaques&al20}, which assume a complete knowledge of the dynamics governing the motion in the form of a physics engine, we rely only on the knowledge of general physical laws, such as, world consists of objects, which have position and velocity. We propose an additional decoder based loss in the pixel space, imposed in a curriculum manner, to further refine the latent space predictions. Experiments in multiple different settings demonstrate that while Kipf et al. model is effective at capturing object interactions, our model can be significantly more effective at localising objects, resulting in improved performance in 3 out of 4 domains that we experiment with. Additionally, our model can learn highly intrepretable feature maps, resembling actual object positions.

==> abstract_1.tex <==
\begin{abstract}
We focus on the task of future frame prediction in video governed by underlying physical dynamics. We work with models which are object-centric, i.e., explicitly work with object representations, and propagate a loss in the latent space. Specifically, our research builds on recent work by Kipf et al.~\cite{kipf&al20}, which predicts the next state via contrastive learning of object interactions in a latent space using a Graph Neural Network. We argue that injecting explicit inductive bias in the model, in form of general physical laws, can help not only make the model more interpretable, but also improve the overall prediction of model. As a natural by-product, our model can spit out position and velocity of various objects, without having any explicit supervision about these motion parameters at the training time. In comparison with earlier works~\cite{jaques&al20}, which assume a complete knowledge of the dynamics governing the motion in the form of a physics engine, we rely only on the knowledge of general physical laws, such as, world consists of objects, which have position and velocity. Finally, we propose an additional decoder based loss in the pixel space, imposed in a curriculum manner, to further improve the latent space predictions. Experiments in multiple different settings demonstrate that our model significantly improves the performance of the Kipf et al. baseline, while also being able to accurately predict the position and velocity of various objects in the underlying video.

\end{abstract}


==> expt_v0.tex <==
\section{Experiments}


% \begin{figure}
%     \centering
%     \begin{subfigure}[b]
%     \centering
%          \includegraphics[scale = 0.7]{images/2o_2m_ready.png}
%          \caption{(2 obj, 2 mov)}
%          \label{fig:2obj_2mov}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]
%     \centering
%          \includegraphics[scale = 0.7]{images/3o_3m_ready.png}
%          \caption{(3 obj, 3 mov)}
%          \label{fig:3obj_3mov}
%     \end{subfigure}
    
%     \vfill
%     \begin{subfigure}[b][0.1\textwidth]
%     \centering
%          \includegraphics[scale = 0.7]{images/collision_ready.png}
%          \caption{Column Collision}
%          \label{fig:collision}
%     \end{subfigure}
%     \hspace{\fill}
%     \begin{subfigure}[b][0.1\textwidth]
%     \centering
%          \includegraphics[scale = 0.7]{images/physics_ready.png}
%          \caption{3 body physics}
%          \label{fig:physics}
%     \end{subfigure}
%     \caption{Test Environments}
%     \label{fig:envs}
% \end{figure}
In this section, we discuss the experiments conducted to provide evidence for the merit of PE-CSWM over the baselines and ... Write 1-2 line intro...

\begin{figure}[htbp]
    \minipage{0.5\linewidth}
      \centering
      \includegraphics[width=\linewidth]{images/2o_2m_ready.png}
      (a) (2 obj, 2 mov)
    \endminipage\hfill
    \minipage{0.5\linewidth}
      \centering
      \includegraphics[width=\linewidth]{images/3o_3m_ready.png}
      (b) (3 obj, 3 mov)
    \endminipage
    \vspace{0.2cm}
    \minipage{0.5\linewidth}%
      \centering
      \includegraphics[width=\linewidth]{images/collision_ready.png}
      (c) Column Collision
    \endminipage
    \minipage{0.4\linewidth}%
      \centering
      \includegraphics[width=\linewidth]{images/physics_ready.png}
      (d) 3 body Physics
    \endminipage
    \caption{\label{Test Environments} Sample observations of our test environments. a-b belong to the Non-Collision environments and c-d belong to Collision Environments. Arrows in c indicate the velocity directions of colliding objects}
\end{figure}

\subsection{Environments}
For the purpose of our experiments, we use broadly two class of environments:
\begin{enumerate}
    \item \textbf{Non-Collision Environments:} These are the environments where there is no collision between the objects in the scene. Objects in these environments are simple shapes like triangles, circles, squares etc. These objects move independently of each other. This class of environments can be generalised as p objects and q moving where $q \in \{0,p\}$ and represented as ($p$ obj, $q$ mov). We use 2 environments from this category viz. (2 obj, 2 mov) and (3 obj, 3 mov). In these environments, each object is constrained to move only in its own respective column with a constant velocity within the frame boundaries. However, the objects bounce off the frame walls and undergo a 180 degree change in their velocity direction, magnitude remaining the same \pscom{*(refer to figure here)}.
    \item \textbf{Collision Environments:} As the name suggests, these environments encompass collision between objects, hence the objects no longer move independently but their movement depends on the position of other objects as well. Within this category of environments, we further take 2 environments to test PE-CSWM. First collision environment is the column collision environment wherein the objects are simple shapes as in non-collision environments but now 2 objects move in the same column thus resulting collisions in that column. The semantics of column collision environment have clearly been described in \pscom{*(refer figure here)}. Second collision environment is 3-body physics which is a more real-world based environment with noise in observations.
\end{enumerate}
Each environment has three datasets viz. train, test and val which have all been collected using random policy. The observations for all the environments are of dimension 50 x 50 x 3  and we also provide one step history while performing experiments on both PE-CSWM and baselines.
\subsection{Experimental Setting and baselines}
We compare the performance of PE-CSWM with CSWM \pscom{*(maybe cite here)} and 3 of the CSWM variants which have been referenced as CSWM\_A, CSWM\_B and CSWM\_AB in subsequent sections, tables and plots. CSWM\_A has the additional negative contrastive loss term over CSWM and its loss function then becomes:
\begin{equation}
    \begin{split}
        L = \hyperref[cswm:loss]{L_{CSWM}} + max(0, \gamma - d(\tilde{z}, \hat{z}_{t+1})
    \end{split}
\end{equation}
The rationale behind creating the variant is to ensure the flow of negative contrastive loss through Graph Neural Network in the backpropagation step. The other variant CSWM\_B has a decoder as a part of the model training process. The CSWM\_AB then merely becomes a combination of CSWM\_A and CSWM\_B. 
\newline \newline
For all the baselines, their variants and our PE-CSWM, we train the models on a total of 275 epochs with a two phase curriculum. The first phase of the curriculum continues till 125 epochs while the second phase then begins after 125 epochs and continues till the end. The limits of phase 1 and phase 2 have been empirically tested for different splits in which we found this split to work the best. For any model, whether PE-CSWM or baselines, decoder, if present, gets trained only in the phase 2 and has no role during phase 1.The training and evaluation for each model has been consistently done using 1 NVIDIA K-40 GPU for a period that ranges between 3-9 hours depending on the model being trained.
\subsection{Evaluation Metrics} 
All set of experiments reported have been evaluated using three different metrics viz. Hits at Rank k (Hits @ k), Mean Reciprocal Rank (MRR) and Decoder Loss, details of which have been described ahead. Note that Hits @ 1 and MRR are the same evaluation metrics as used by the CSWM paper. 
\begin{enumerate}
        \item \textbf{Hits @ k :} Hits @ k is a ranking-based metric which provides a means to evaluate the performance of the model directly in the latent space. For the purpose of our experiments, we use k as 1. PE-CSWM gives the predicted encoded representation of the next state i.e. $\hat{z}_{t+1}= z_t + \Delta z_t$. Hits @ 1 measures how close is this $\hat{z}_{t+1}$ to the latent space representation of $s_{t+1}$ i.e. $z_{t+1}$ relative to the encoded representations of the set of reference states sampled randomly from the experience buffer. 
    \item \textbf{Mean Reciprocal Rank (MRR) :} MRR is another ranking-based metric that operated directly on latent state representations and helps assess their quality. MRR is essentially the mean of the reciprocal of rank of the predicted next state encoded representation, $\hat{z}_{t+1}$ amongst the other randomly chosen reference states based on their squared euclidean distance to the latent space representation of $s_{t+1}$ i.e. $z_{t+1}$. Mathematically, MRR is given by: 
\[MRR =  \frac{1}{N} \sum_{n=1}^{N} \frac{1}{rank_{n}} \]
    \item \textbf{Decoder Loss :} Decoder loss is essentially the binary cross entropy loss between the $\hat{s}_{n}$ and $s_{n}$ where the time step n can be anywhere from t + 1 to t + 99 for the purpose of our experiments and t is the current time step. This helps us to evaluate the quality of the pixel-based reconstruction using only the latent space representation of the state and indirectly also comments upon the quality of underlying representation.
    \item \textbf{Position Accuracy :}
    \item \textbf{Velocity Accuracy :}
\end{enumerate}
\subsection{Qualitative Results}
\subsection{Quantitative Results}
Hello!
\begin{figure*}[h]
\includegraphics[scale = 0.6]{images/2o_2m_our_variants.png}
\label{fig:2o_2m_our_variants}
\caption{Comparison between performance of PE-CSWM\_C, PE-CSWM\_D and PE-CSWM on Hits @ 1(Higher is better), MRR (Higher is better) and Decoder Loss (Lower is better). Environment here is (2 obj, 2 mov)}
\end{figure*}

\begin{figure*}[h]
\begin{center}
    \includegraphics[scale = 0.6]{images/2o_2m_baseline_variants.png}
\end{center}
\label{fig:2o_2m_baseline_variants}
\caption{Comparison between performance of CSWM ,CSWM\_A, CSWM\_B, CSWM\_AB, PE-CSWM\_C and PE-CSWM on Hits @ 1(Higher is better) and MRR (Higher is better). Environment here is (2 obj, 2 mov)}
\end{figure*}

\begin{figure*}[h]
\includegraphics[scale = 0.6]{images/3o_3m_our_variants.png}
\label{fig:3o_3m_our_variants}
\caption{Comparison between performance of PE-CSWM\_C, PE-CSWM\_D and PE-CSWM on Hits @ 1(Higher is better), MRR (Higher is better) and Decoder Loss (Lower is better). Environment here is (3 obj, 3 mov)}
\end{figure*}

\begin{figure*}[h]
\begin{center}
    \includegraphics[scale = 0.6]{images/3o_3m_baseline_variants.png}
\end{center}
\label{fig:3o_3m_baseline_variants}
\caption{Comparison between performance of CSWM ,CSWM\_A, CSWM\_B, CSWM\_AB, PE-CSWM\_C and PE-CSWM on Hits @ 1(Higher is better) and MRR (Higher is better). Environment here is (3 obj, 3 mov)}
\end{figure*}

\begin{figure*}[h]
\includegraphics[scale = 0.6]{images/collision_our_variants.png}
\label{fig:column_collision_our_variants}
\caption{Comparison between performance of PE-CSWM\_C, PE-CSWM\_D and PE-CSWM on Hits @ 1(Higher is better), MRR (Higher is better) and Decoder Loss (Lower is better). Environment here is column collision}
\end{figure*}

\begin{figure*}[h]
\begin{center}
    \includegraphics[scale = 0.6]{images/collision_baseline_variants.png}
\end{center}
\label{fig:column_collision_baseline_variants}
\caption{Comparison between performance of CSWM ,CSWM\_A, CSWM\_B, CSWM\_AB, PE-CSWM\_C and PE-CSWM on Hits @ 1(Higher is better) and MRR (Higher is better). Environment here is column collision}
\end{figure*}



\subsection{Ablation Study}


==> results.tex <==

%\section{Results and plots}



%%Qualitative Results
% \begin{figure*}[h]
% \begin{center}
% \includegraphics[scale = 0.6]{images/dc_d_i_c_2o_2m.png}
% \end{center}
% \label{fig:column_collision_our_variants}
% \caption{Comparison between performance of ICSWM + D - C, ICSWM, ICSWM + D and CSWM on Hits @ 1(Higher is better) and MRR (Higher is better). Environment here is 3 Body Physics}
% \end{figure*}

